Characterizing User Behavior: The Interplay Between Mobility Patterns and Mobile Traffic

Mobile devices have become essential for capturing human activity, and eXtended Data Records (XDRs) offer rich opportunities for detailed user behavior modeling, which is useful for designing personalized digital services. Previous studies have primarily focused on aggregated mobile traffic and mobility analyses, often neglecting individual-level insights. This paper introduces a novel approach that explores the dependency between traffic and mobility behaviors at the user level. By analyzing 13 individual features that encompass traffic patterns and various mobility aspects, we enhance the understanding of how these behaviors interact. Our advanced user modeling framework integrates traffic and mobility behaviors over time, allowing for fine-grained dependencies while maintaining population heterogeneity through user-specific signatures. Furthermore, we develop a Markov model that infers traffic behavior from mobility and vice versa, prioritizing significant dependencies while addressing privacy concerns. Using a week-long XDR dataset from 1,337,719 users across several provinces in Chile, we validate our approach, demonstrating its robustness and applicability in accurately inferring user behavior and matching mobility and traffic profiles across diverse urban contexts.

==> related_works.tex <==
Mobile traffic data and human mobility data each provide unique insights into human activity. % valuable for many applications
While often studied separately, their strong interrelation has been demonstrated in various research. This section reviews the state-of-the-art studies on both data types and examines existing research on their correlation.

\vspace{0.13cm}
\noindent \textbf{Human Mobility data.} Human mobility is a well-researched area with significant value across several fields, including public health, sociology, transportation, and tourism~\cite{DeDomenico:2013, Koszowski:2019}. 
Studies have examined it from multiple angles, identifying key laws that govern movements~\cite{Gonzalez:2008, Rhee:2011} and creating models for simulating~\cite{Keramat:2016}, predicting~\cite{Wang_Jinzhong:2019}, and generating~\cite{Kobayashi:2023} mobility patterns at various scales. 
%It has been extensively characterized from multiple perspectives highlighting the fundamental laws governing it~\cite{Gonzalez:2008, Rhee:2011} to facilitate the development of models for simulating~\cite{Keramat:2016}, predicting~\cite{Wang_Jinzhong:2019}, and generating~\cite{Kobayashi:2023} human mobility at various scales. 
%using advanced techniques such as generative AI. By analyzing these aspects, researchers aim to capture and model the complexities of human movement, allowing for more accurate predictions and simulations of mobility patterns.It has been characterized from various perspectives to understand, model, simulate, predict, and generate it using generative machine learning algorithms.
%\\ Human mobility can be examined at both the individual level (i.e., individual mobility) and the group level (i.e., flows). While group mobility provides global insights into human dynamics during mobility, 
When analyzed at an individual level, human mobility provides more detailed insights by accounting for personal differences.
%accounting for the heterogeneity of each person within the overall trend . In this context, several studies agree that 
Research shows that individuals exhibit varied behaviors in their movement patterns~\cite{Pappalardo:2015, Scherrer:2018} %. Recent research~\cite{Amichi:2020} 
with a recent study~\cite{Amichi:2020} identifying three mobility profiles
%based on visitation regularity and distinct temporal, spatial, and social patterns: 
(i) \textit{Scouters}, more inclined to explore and discover new areas; (ii) \textit{Routiners}, who maintain a steady routine and rarely break their established patterns%, preferring to stay within familiar places
; and (iii) \textit{Regulars}, with a moderate behavior balancing between explorations and revisits. 
%with frequent returns compared to Scouters but have distinctly smaller intermittencies than Routiners, constantly alternating between exploration and revisits.

\vspace{0.13cm}
\noindent \textbf{Mobile Traffic data} captures daily user activity on cellular networks valuable for tasks like network optimization and resource management. This study focuses on XDR traces, extensively studied in the literature for characterization, prediction~\cite{Aceto:2021, Trinh:2017, Wu_Jing:2018}, or generation~\cite{Kouam:2023} purposes.
%which reflect user behavior through data volume generated during activities such as work, navigation, and streaming.
%Extensively studied in the literature for characterization and prediction~\cite{Aceto:2021, Trinh:2017, Wu_Jing:2018}, XDR data is sometimes generated synthetically using deep learning to cope with the related privacy constraints~\cite{Kouam:2023}. 
Similar to human mobility data, individual-level analyses reveal distinct user profiles in data generation~\cite{Naboulsi:2014, Jing:2018, Eduardo:2015}. \cite{Eduardo:2015} distinguishes four profiles: \textit{Light Occasional (LO), Light Frequent (LF), Heavy Occasional (HO), and Heavy Frequent (HF)}. Light users generate up to 20GB per day, while Heavy users exceed this amount. "Occasional" and "Frequent" distinctions depend on the number of sessions users generate daily.

\vspace{0.13cm}
\noindent \textbf{Mobility and Traffic data dependency.}
Several studies have demonstrated the close relationship between mobile traffic and human mobility through statistical correlations \cite{Chen:2015, Wang:2019, Xu:2017, Alipour:2018, Merkebe:2013, Paul:2011}. The movement patterns of mobile network users—shaped by daily routines, points of interest, and behaviors—introduce significant temporal and spatial dynamics into mobile traffic data, which are crucial for understanding, modeling, and predicting cellular traffic at both large and fine scales. Additionally, the prevalence of network events among dispersed urban populations provides rich datasets that reflect underlying mobility patterns and urban dynamics, which are essential for effective city management and planning.

Existing studies on the correlation between mobility and mobile traffic have primarily focused on the city scale. For instance, \cite{Xu_Kai:2021} examined the geographic distribution of cellular traffic and uncovered strong spatiotemporal dependencies, while \cite{Chen:2015} identified spatial inhomogeneities in traffic patterns between urban and rural areas. Similarly, \cite{Merkebe:2013} illustrated how mobile traffic data can reveal city dynamics and infrastructure usage. However, while these studies offer valuable insights, they do not fully address the correlation between traffic and mobility at the individual level. Some works, such as \cite{Alipour:2018}, explored mobility-traffic correlations in WLAN settings at the device level, categorizing devices as "cellos" (stationary) and "flutes" (mobile), and found that cellos generated traffic more frequently, albeit in smaller volumes. Similarly, \cite{Paul:2011} investigated the relationship between subscriber mobility and traffic generation in 3G networks, concluding that more mobile users produced higher traffic volumes. %Despite these advancements, more detailed profiling of individual behavior remains largely unexamined, underscoring the need for further research into fine-grained traffic-mobility inference models.
While these approaches provide a preliminary understanding of how mobility correlates with traffic, a more detailed examination of the traffic-mobility interrelation at the individual behavior level remains largely unexplored, limiting the flexibility and potential of individual behavior profiling.

\vspace{0.13cm} \noindent \textbf{Positioning.} This paper introduces a novel approach that establishes a direct dependency between traffic and mobility behavior at the individual level. We explore the implications of this dependency for flexible user behavior modeling and the accurate inference of behavioral patterns in mobile networks.

